Non-Fickian single-file pore transport

Single file diffusion (SFD) exhibits anomalously slow collective transport when particles are able to immobilize by binding and unbinding to the one-dimensional channel within which the particles diffuse. We have explored this system for short pore-like channels using a symmetric exclusion process (SEP) with fully stochastic dynamics. We find that for shorter channels, a non-Fickian regime emerges for slow binding kinetics. In this regime the average flux $\langle \Phi \rangle \sim 1/L^3$, where $L$ is the channel length in units of the particle size. We find that a two-state model describes this behavior well for sufficiently slow binding rates, where the binding rates determine the switching time between high-flux bursts of directed transport and low-flux leaky states. Each high-flux burst is Fickian with $\langle \Phi \rangle \sim 1/L$. Longer systems are more often in a low flux state, leading to the non-Fickian behavior.

==> PoreSFD (1)/cutouts.tex <==
%HERE change
Most SFD studies are either concerned with the statistics of tracer particle subdiffusion, or with the characterization of average transport in long channels. The exception is in pore-transport studies, both experimental and molecular dynamics (MD) investigations.  The mechanism of our flux switching is quite distinctive, and applies to pores that are partially occupied or that do not have hydrogen bonding networks. 

Biological pores have unscreened charges that strongly interact with SFD water within them.

% switching effects (and observing)
While agreement on the magnitude of the effect is suggestive, we can predict that current fluctuations at the scale of $10^7/s$ would be associated with the effect. This would require unprecedented precision in experimental studies (but perhaps possible) or in MD studies.

We do not include possible alternative mechanisms such as gated channel entry or hydrogen bonding between water molecules, which lets us examine how interactions between diffusing particles and channel walls can affect transport through pores.

The scale of our non-Fickian effects with channel length are similar to those reported in nano-scale biological water channels.



%Similar considerations seem to rule out strong non-Fickian effects in  molecular dynamics (MD) simulations of SFD of simple molecules such as water \cite{Fang2008}. For water transport in CNT Hummer et al. \cite{Hummer2001} reported pulse-like transport. However, this was limited to full occupancy of the CNT interior and ascribed to collective reversals of the hydrogen bonding chain within the CNT. 

Transient particle immobility has been considered within coarse-grained models of SFD pore transport with an external drive \cite{Piasecki2004} or with blocking only at one pore end \cite{Bauer2006}. For these cases, we do not expect (and they do not report) the anomalous length dependence that we describe due to the external drive, the small number of binding sites, and the coarse-grained approaches. 

% journal PRE Letter
% refs 
% T Chou (UCLA)
% E Frey (Munich)
% PL Krapivsky (Boston)
% Kirone Mallick (Saclay)


==> cutouts.tex <==
%HERE change
Most SFD studies are either concerned with the statistics of tracer particle subdiffusion, or with the characterization of average transport in long channels. The exception is in pore-transport studies, both experimental and molecular dynamics (MD) investigations.  The mechanism of our flux switching is quite distinctive, and applies to pores that are partially occupied or that do not have hydrogen bonding networks. 

Biological pores have unscreened charges that strongly interact with SFD water within them.

% switching effects (and observing)
While agreement on the magnitude of the effect is suggestive, we can predict that current fluctuations at the scale of $10^7/s$ would be associated with the effect. This would require unprecedented precision in experimental studies (but perhaps possible) or in MD studies.

We do not include possible alternative mechanisms such as gated channel entry or hydrogen bonding between water molecules, which lets us examine how interactions between diffusing particles and channel walls can affect transport through pores.

The scale of our non-Fickian effects with channel length are similar to those reported in nano-scale biological water channels.



%Similar considerations seem to rule out strong non-Fickian effects in  molecular dynamics (MD) simulations of SFD of simple molecules such as water \cite{Fang2008}. For water transport in CNT Hummer et al. \cite{Hummer2001} reported pulse-like transport. However, this was limited to full occupancy of the CNT interior and ascribed to collective reversals of the hydrogen bonding chain within the CNT. 

Transient particle immobility has been considered within coarse-grained models of SFD pore transport with an external drive \cite{Piasecki2004} or with blocking only at one pore end \cite{Bauer2006}. For these cases, we do not expect (and they do not report) the anomalous length dependence that we describe due to the external drive, the small number of binding sites, and the coarse-grained approaches. 

% journal PRE Letter
% refs 
% T Chou (UCLA)
% E Frey (Munich)
% PL Krapivsky (Boston)
% Kirone Mallick (Saclay)

